Intersectionality in Conversational AI Safety: How Bayesian Multilevel Models Help Understand Diverse Perceptions of Safety

Conversational AI systems exhibit a level of human-like behavior that promises to have profound impacts on many aspects of daily life -- how people access information, create content, and seek social support. Yet these models have also shown a propensity for biases, offensive language, and conveying false information. Consequently, understanding and moderating safety risks in these models is a critical technical and social challenge. Perception of safety is intrinsically subjective, where many factors -- often intersecting -- could determine why one person may consider a conversation with a chatbot safe and another person could consider the same conversation unsafe. In this work, we focus on demographic factors that could influence such diverse perceptions. To this end, we contribute an analysis using Bayesian multilevel modeling to explore the connection between rater demographics and how raters report safety of conversational AI systems. We study a sample of 252 human raters stratified by gender, age group, race/ethnicity group, and locale. This rater pool provided safety labels for 1,340 human-chatbot conversations. Our results show that intersectional effects involving demographic characteristics such as race/ethnicity, gender, and age, as well as content characteristics, such as degree of harm, all play significant roles in determining the safety of conversational AI systems. For example, race/ethnicity and gender show strong intersectional effects, particularly among South Asian and East Asian women. We also find that conversational degree of harm impacts raters of all race/ethnicity groups, but that Indigenous and South Asian raters are particularly sensitive to this harm. Finally, we observe the effect of education is uniquely intersectional for Indigenous raters, highlighting the utility of multilevel frameworks for uncovering underrepresented social perspectives.

==> unused.tex <==
We define safety along four major dimensions: \emph{harmful content}, \emph{unfair bias} , \emph{misinformation}, and \emph{political affiliation}. In the case of misinformation, a rater's perception of safety depends on what the rater knows. With respect to unfair bias, in order to avoid censorship, offensive speech is often deliberately obscured by the speaker, in a ``dogwhistle'' fashion, so that a message may send a clear signal of unfair bias to those who are aware of it, but may appear innocuous to others \cite{sang_origin_2022}. Demographics often plays a major role in how many subjective issues are perceived.

In this paper, we focus on the role that demographics play in determining how human raters evaluate machine-generated dialogues for safety. With the growing power of machine-learning-based intelligent systems---and with it the increased role such systems promise to play in our lives---the need for evaluation frameworks that are fair to all cross-sections of society is increasingly important. A major challenge has been that demographic factors are complex, and may interact with each other in unexpected ways. 

We explore the following research questions.
\begin{description}
\item[RQ1.] What is the best model for predicting how human raters report safety risks in chatbot conversations, based on their demographic affiliations?
\item[RQ2.] Which demographic properties are most predictive of how human raters report safety risks in chatbot conversations?
\end{description}

 a class of models that substantially overlaps with MLMs, though our multilevel models are nonlinear and thus more sophisticated than theirs; the authors did not specify whether their models were Bayesian or not)
 
 
 We report these results in two ways. First, Tables \ref{tab:phase} and \ref{tab:expert} show estimated odds according to the model for the class in question versus the variable's reference class that the dialogue being rated \emph{safe}. Note that, for gender \emph{Man} is the reference class, for race it is \emph{White}, for Phase it is \emph{Phase 1}, and for age it is \emph{Gen Z}. The tables are comprehensive, except that we omit results for the  \emph{Nonbinary} and the \emph{Other gender} raters because there was only one of each.  
 
 The estimates for Intercept[1] and Intercept[2] represent the reference group probability thresholds among the three ordinal rating categories: safe, unsure, unsafe. Thus, Intercept[1] indicates the default odds of selecting unsure over safe and Intercept[2] indicates the default odds of selecting unsafe over safe. These intercept terms allow one to calculate safety ratings for the average rater according to unique combinations of demographic variables. For instance, to determine the odds that a rater--who is Asian, a woman, college-educated, and millenial--rates a dialogue as unsafe compared to the average college-educated, Gen Z, White man, one would multiply Intercept[2] by the estimates for Asian, Woman, Age.L, Asian:Woman, and Asian:Agel.L. Unlike standard confidence intervals, Bayesian credible intervals are much more intuitive to interpret. Our reported 95\% credible intervals, for instance, show that, based on the data observed, there is a 95\% probability that the true population estimate falls within the interval.
 
 Second, Figures \ref{fig:race_gender}--\ref{fig:race_genz} show credible intervals for the estimated likelihood of reporting unsafe for select variables. Unlike the tables, these figures report results for all classes, including the reference classes.
 
 Our results for the largest model that includes expert ratings for demographic predictors of rater behavior for safety, i.e., Q\_overall $\sim$ race $*$ (gender $+$ age $+$ phase) $+$ education $+$ (1 $|$ rater\_id) $+$ (1 $|$ dialogue\_id), according to the R notation that is standard for specifying MLMs, is shown in Table \ref{tab:expert}. This model tests the interaction of race with gender, age, phase. Education is an additional covariate. 


The model shows that younger raters perceive more unsafety compared to older raters (Figure \ref{fig:race_genx}). Note the very large ordinal effect. There were substantially lower reports of safety for Phase Three versus Phase two content.

%Intersectional effects for Asian and Indian women: 
Compared to the difference between White men and women, Asian women perceive substantially more safety across dialogues than Asian men (Figure \ref{fig:race_gender}).
Compared to the difference between White men and women, Indian women perceive substantially less safety than Indian men (Figure \ref{fig:race_gender}).

The age effect is softer for Asian raters, compared to White raters: as age increases, perceptions of safety risks do not decrease as much as we see for White raters (Figure \ref{fig:race_gender})
Another way to look at this: the age difference in ratings seems more pronounced for White raters compared to raters of color (holding all other factors constant; (Figure \ref{fig:race_gender})

The large odds for race in every variable (Tables \ref{tab:phase} and \ref{tab:expert}) suggests that White (the reference class for race) raters are much more likely than other raters to report a dialogue as \emph{safe}. The effects representing V1 vs. V3 differences in safety ratings compared to White raters are LARGE for most non-White raters (Figure \ref{fig:race_phase}).

Table \ref{tab:expert} shows the results of our largest model that \textbf{DID} include expert ratings, i.e., Q\_overall $\sim$ race $*$ (gender $+$ age $+$ degree\_of\_harm) $+$ education $+$ (1 $|$ rater\_id) $+$ (1 $|$ dialogue\_id), according to standard R notation. This model tests race’s interaction with gender, age, and degree\_of\_harm, according to our expert's ratings. Education is an additional covariate. It shows that that our expert-annotated degree of harm positively relates to perceptions of safety. For Black, Indian, Indigenous and Latine raters (compared to White raters), we can be strongly confident that harmful content (slightly) relates to perceptions of safety. In other words, these rater groups' perceptions of safety are more influenced by extreme content compared to White raters.

\section{Greg's Rephrasing of Results}

Our results support a number of conclusions about our research questions. 

Our motivation behind considering Phase separately from expert ratings of severity was to investigate whether the Phase can act as a ``stand-in'' of sorts for the experts, because the dialogues in Phases 1 and 2 were rated \emph{safe} more frequently than those in Phase 3. The rather stark difference in model performance between expert and ratings-as-a-variable-based models suggests that severity and Phase are not comparable as independent variables.

Regarding the non-intersectional aspects of RQ2, raters are more likely to report harm if they are White or older. Women were also more likely to report harm, but the effect is smaller in gender than in race or age. 

Some effects could only be observed by taking the interaction of two demographic variables into account. In particular, the effect of age on safety reported is lessened for Asian raters compared to .... 

\begin{comment}
\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/gender.png}
    \caption{Credible intervals for the AD linear described in the \emph{Methods} section show that men are more sensitive to safety risks than women.}
    \label{fig:gender}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/age.png}
    \caption{Credible intervals for the AD linear Bayesian multilevel model described in Section \ref{sec:methods}  show that older raters are less sensitive to safety risks that younger raters.}
    \label{fig:age}
\end{figure}
\end{comment}

% OLD Table of QS Models
% Degree of Harm Models Table
% Shows odds ratios instead
%\clearpage
%\onecolumn
\begin{table}
\tiny
\begin{tabular}{ldddd}
\toprule
  & {Model 1} & {Model 2} & {Model 3} & {Model 4}\\
\midrule
Intercept[1] & 1.470 & 2.415 & 2.428 & 2.151\\
 & {}[1.305, 1.669] & {}[1.797, 3.244] & {}[1.807, 3.234] & {}[1.550, 2.989]\\
Intercept[2] & 1.866 & 3.110 & 3.131 & 2.774\\
 & {}[1.656, 2.118] & {}[2.313, 4.175] & {}[2.326, 4.171] & {}[1.995, 3.849]\\
Asian & {} & 0.590 & 0.636 & 1.298\\
 & {} & {}[0.401, 0.850] & {}[0.439, 0.923] & {}[0.740, 2.236]\\
Black & {} & 1.204 & 1.294 & 1.233\\
 & {} & {}[0.804, 1.781] & {}[0.879, 1.875] & {}[0.704, 2.141]\\
Indian & {} & 3.113 & 3.157 & 1.766\\
 & {} & {}[2.228, 4.359] & {}[2.279, 4.524] & {}[1.130, 2.796]\\
Indigenous & {} & 2.437 & 2.494 & 2.044\\
 & {} & {}[1.307, 4.682] & {}[1.300, 4.669] & {}[0.906, 4.711]\\
Latine & {} & 1.452 & 1.404 & 1.410\\
 & {} & {}[0.749, 2.747] & {}[0.738, 2.662] & {}[0.446, 4.849]\\
Multiracial & {} & 1.386 & 1.453 & 1.410\\
 & {} & {}[0.796, 2.427] & {}[0.849, 2.464] & {}[0.671, 3.008]\\
RaceOther & {} & 1.591 & 1.685 & 1.663\\
 & {} & {}[0.785, 3.175] & {}[0.874, 3.357] & {}[0.736, 3.832]\\
Nonbinary & {} & 0.790 & 0.870 & 0.923\\
 & {} & {}[0.180, 3.099] & {}[0.217, 3.401] & {}[0.149, 5.429]\\
Self-Described & {} & 0.977 & 0.992 & 0.980\\
 & {} & {}[0.038, 25.238] & {}[0.042, 19.715] & {}[0.042, 21.433]\\
Woman & {} & 1.247 & 1.230 & 1.163\\
 & {} & {}[0.959, 1.628] & {}[0.954, 1.582] & {}[0.771, 1.727]\\
Age.L & {} & 0.723 & 0.734 & 0.551\\
 & {} & {}[0.638, 0.819] & {}[0.646, 0.835] & {}[0.442, 0.689]\\
Severity.L & {} & 1.575 & 1.592 & 1.482\\
 & {} & {}[1.402, 1.777] & {}[1.396, 1.813] & {}[1.281, 1.713]\\
Highschoolorbelow & {} & 1.219 & 1.108 & 0.929\\
 & {} & {}[0.889, 1.699] & {}[0.803, 1.559] & {}[0.670, 1.304]\\
EducationOther & {} & 0.461 & 0.448 & 0.949\\
 & {} & {}[0.282, 0.750] & {}[0.271, 0.732] & {}[0.514, 1.735]\\
Asian:Woman & 0.485\\
 & {}[0.240, 0.969]\\
Black:Woman & 0.858\\
 & {}[0.417, 1.766]\\
Indian:Woman & 1.668\\
 & {}[0.926, 3.030]\\
Indigenous:Woman & 1.210\\
 & {}[0.403, 3.759]\\
Latine:Woman & 1.276\\
 & {}[0.396, 4.049]\\
Multiracial:Woman & 1.134\\
 & {}[0.419, 3.038]\\
RaceOther:Woman & 0.905\\
 & {}[0.291, 2.799]\\
Asian:Age.L & 1.657\\
 & {}[1.256, 2.193]\\
Black:Age.L & 1.589\\
 & {}[0.857, 2.958]\\
Indian:Age.L & 1.280\\
 & {}[0.859, 1.980]\\
Indigenous:Age.L & 1.633\\
 & {}[0.540, 5.320]\\
Latine:Age.L & 0.901\\
 & {}[0.126, 6.249]\\
Multiracial:Age.L & 1.186\\
 & {}[0.471, 2.975]\\
RaceOther:Age.L & 1.189\\
 & {}[0.357, 4.029]\\
Asian:Severity.L & 1.036\\
 & {}[0.897, 1.200]\\
Black:Severity.L & 0.986\\
 & {}[0.869, 1.117]\\
Indian:Severity.L & 1.096\\
 & {}[0.966, 1.247]\\
Indigenous:Severity.L & 1.259\\
 & {}[1.033, 1.529]\\
Latine:Severity.L & 1.151\\
 & {}[0.901, 1.463]\\
Multiracial:Severity.L & 1.009\\
 & {}[0.848, 1.203]\\
RaceOther:Severity.L & 0.889\\
 & {}[0.674, 1.175]\\
sd\_convers\_id\_\_Inter & 2.215 & 2.064 & 2.073 & 2.075\\
 & {}[2.116, 2.323] & {}[1.984, 2.161] & {}[1.989, 2.173] & {}[1.988, 2.171]\\
sd\_rater\_id\_\_Intercept & 2.302 & 2.429 & 2.402 & 2.344\\
 & {}[2.140, 2.511] & {}[2.201, 2.728] & {}[2.179, 2.701] & {}[2.134, 2.616]\\
sd\_rater\_id\_\_Sever.L & {} & {} & 1.170 & 1.167\\
 & {} & {} & {}[1.111, 1.235] & {}[1.106, 1.233]\\
cor\_rater\_id\_Inter\_\_Sever.L & {} & {} & 1.013 & 0.993\\
 & {} & {} & {}[0.742, 1.384] & {}[0.718, 1.380]\\
%\midrule
%Num.Obs. & 56468 & 42148 & 42148 & 42148\\
%R2 & 0.378 & 0.380 & 0.384 & 0.385\\
%R2 Marg. & 0.000 & 0.130 & 0.127 & 0.135\\
%ICC & 0.6 & {} & {} & {}\\
%ELPD & -35303.1 & -26553.5 & -26514.2 & -26509.1\\
%ELPD s.e. & 178.4 & 154.5 & 154.6 & 154.8\\
%LOOIC & 70606.2 & 53107.1 & 53028.5 & 53018.1\\
%LOOIC s.e. & 356.8 & 309.0 & 309.1 & 309.6\\
%WAIC & 70602.7 & 53103.1 & 53023.0 & 53012.4\\
\end{tabular}
\caption{Summary of Results for MLMs with Expert-Annotated Data.}
\end{table}

% FINAL Table of Models of QS Dataset
\begin{table}
\centering
\begin{tabular}[t]{lddd}
\toprule
  & {QS Model 1} & {QS Model 2.0} & {QS Model 2.1}\\
\midrule
Intercept[1] & 1.470 & 2.415 & 2.428\\
 & {}[1.305, 1.669] & {}[1.797, 3.244] & {}[1.807, 3.234]\\
Intercept[2] & 1.866 & 3.110 & 3.131\\
 & {}[1.656, 2.118] & {}[2.313, 4.175] & {}[2.326, 4.171]\\
RaceEastAsian & {} & 0.590 & 0.636\\
 & {} & {}[0.401, 0.850] & {}[0.439, 0.923]\\
RaceBlack & {} & 1.204 & 1.294\\
 & {} & {}[0.804, 1.781] & {}[0.879, 1.875]\\
RaceSouthAsian & {} & 3.113 & 3.157\\
 & {} & {}[2.228, 4.359] & {}[2.279, 4.524]\\
RaceIndigenous & {} & 2.437 & 2.494\\
 & {} & {}[1.307, 4.682] & {}[1.300, 4.669]\\
RaceLatine & {} & 1.452 & 1.404\\
 & {} & {}[0.749, 2.747] & {}[0.738, 2.662]\\
RaceMultiracial & {} & 1.386 & 1.453\\
 & {} & {}[0.796, 2.427] & {}[0.849, 2.464]\\
RaceOther & {} & 1.591 & 1.685\\
 & {} & {}[0.785, 3.175] & {}[0.874, 3.357]\\
GenderNonbinary & {} & 0.790 & 0.870\\
 & {} & {}[0.180, 3.099] & {}[0.217, 3.401]\\
GenderSelf-Described & {} & 0.977 & 0.992\\
 & {} & {}[0.038, 25.238] & {}[0.042, 19.715]\\
GenderWoman & {} & 1.247 & 1.230\\
 & {} & {}[0.959, 1.628] & {}[0.954, 1.582]\\
Age.L & {} & 0.723 & 0.734\\
 & {} & {}[0.638, 0.819] & {}[0.646, 0.835]\\
Severity.L & {} & 1.575 & 1.592\\
 & {} & {}[1.402, 1.777] & {}[1.396, 1.813]\\
EducationHighschoolorbelow & {} & 1.219 & 1.108\\
 & {} & {}[0.889, 1.699] & {}[0.803, 1.559]\\
EducationOther & {} & 0.461 & 0.448\\
 & {} & {}[0.282, 0.750] & {}[0.271, 0.732]\\
sd\_dialogue\_id\_\_Intercept & 2.215 & 2.064 & 2.073\\
 & {}[2.116, 2.323] & {}[1.984, 2.161] & {}[1.989, 2.173]\\
sd\_rater\_id\_\_Intercept & 2.302 & 2.429 & 2.402\\
 & {}[2.140, 2.511] & {}[2.201, 2.728] & {}[2.179, 2.701]\\
sd\_rater\_id\_\_Severity.L & {} & {} & 1.170\\
 & {} & {} & {}[1.111, 1.235]\\
cor\_rater\_id\_\_Intercept\_\_Severity.L & {} & {} & 1.013\\
 & {} & {} & {}[0.742, 1.384]\\
\bottomrule
\end{tabular}
\caption{Summary of Results for MLMs with Expert-Annotated Data.}
\end{table}

% OLD table of AD model
\begin{table}
\tiny
\centering
\begin{tabular}[t]{lddd}
\toprule
  & {Model 1} & {Model 2} & {Model 3}\\
\midrule
Intercept[1] & 2.053 & 3.739 & 3.037\\
 & {}[1.845, 2.304] & {}[2.755, 5.065] & {}[2.221, 4.198]\\
Intercept[2] & 2.615 & 4.819 & 3.915\\
 & {}[2.348, 2.934] & {}[3.551, 6.525] & {}[2.860, 5.404]\\
Asian & {} & 0.529 & 0.985\\
 & {} & {}[0.364, 0.765] & {}[0.489, 1.966]\\
Black & {} & 1.141 & 0.826\\
 & {} & {}[0.783, 1.700] & {}[0.480, 1.432]\\
Indian & {} & 3.077 & 1.256\\
 & {} & {}[2.174, 4.389] & {}[0.812, 1.950]\\
Indigenous & {} & 2.272 & 1.436\\
 & {} & {}[1.235, 4.229] & {}[0.611, 3.442]\\
Latine & {} & 1.283 & 0.937\\
 & {} & {}[0.886, 1.859] & {}[0.554, 1.566]\\
Multiracial & {} & 1.328 & 1.628\\
 & {} & {}[0.763, 2.371] & {}[0.510, 6.072]\\
RaceOther & {} & 1.666 & 2.760\\
 & {} & {}[0.844, 3.296] & {}[0.964, 8.811]\\
%Nonbinary & {} & 0.875 & 0.977\\
% & {} & {}[0.218, 3.435] & {}[0.147, 5.917]\\
%GenderSelf-Described & {} & 0.291 & 0.480\\
% & {} & {}[0.221, 0.382] & {}[0.080, 2.720]\\
Woman & {} & 1.250 & 1.226\\
 & {} & {}[0.977, 1.590] & {}[0.840, 1.801]\\
Age.L & {} & 0.666 & 0.650\\
 & {} & {}[0.606, 0.736] & {}[0.548, 0.771]\\
EducationHighschoolorbelow & {} & 1.313 & 1.148\\
 & {} & {}[0.950, 1.783] & {}[0.846, 1.558]\\
EducationOther & {} & 0.534 & 0.688\\
 & {} & {}[0.350, 0.819] & {}[0.373, 1.255]\\
Phase2 & {} & 0.849 & 0.692\\
 & {} & {}[0.770, 0.935] & {}[0.606, 0.792]\\
Phase3 & {} & 1.771 & 1.418\\
 & {} & {}[1.531, 2.047] & {}[1.179, 1.705]\\
%Asian:Nonbinary & {} & {} & 0.994\\
% & {} & {} & {}[0.041, 25.005]\\
%Black:Nonbinary & {} & {} & 1.016\\
% & {} & {} & {}[0.041, 21.451]\\
%Indian:Nonbinary & {} & {} & 1.001\\
% & {} & {} & {}[0.044, 25.521]\\
%Indigenous:Nonbinary & {} & {} & 0.975\\
% & {} & {} & {}[0.151, 6.657]\\
%Latine:Nonbinary & {} & {} & 1.000\\
% & {} & {} & {}[0.038, 23.747]\\
%Multiracial:Nonbinary & {} & {} & 1.007\\
% & {} & {} & {}[0.042, 27.508]\\
%RaceOther:Nonbinary & {} & {} & 0.987\\
% & {} & {} & {}[0.044, 25.422]\\
%Asian:GenderSelf-Described & {} & {} & 1.005\\
% & {} & {} & {}[0.040, 22.238]\\
%Black:GenderSelf-Described & {} & {} & 1.025\\
% & {} & {} & {}[0.041, 24.157]\\
%Indian:GenderSelf-Described & {} & {} & 1.013\\
% & {} & {} & {}[0.038, 24.477]\\
%Indigenous:GenderSelf-Described & {} & {} & 0.991\\
% & {} & {} & {}[0.041, 26.705]\\
%Latine:GenderSelf-Described & {} & {} & 0.481\\
% & {} & {} & {}[0.082, 2.830]\\
%Multiracial:GenderSelf-Described & {} & {} & 1.005\\
% & {} & {} & {}[0.039, 26.928]\\
%RaceOther:GenderSelf-Described & {} & {} & 0.974\\
% & {} & {} & {}[0.048, 19.841]\\
Asian:Woman & {} & {} & 0.457\\
 & {} & {} & {}[0.232, 0.875]\\
Black:Woman & {} & {} & 0.785\\
 & {} & {} & {}[0.388, 1.567]\\
Indian:Woman & {} & {} & 1.654\\
 & {} & {} & {}[0.931, 2.942]\\
Indigenous:Woman & {} & {} & 1.046\\
 & {} & {} & {}[0.327, 3.413]\\
Latine:Woman & {} & {} & 0.907\\
 & {} & {} & {}[0.487, 1.724]\\
Multiracial:Woman & {} & {} & 0.982\\
 & {} & {} & {}[0.363, 2.685]\\
RaceOther:Woman & {} & {} & 0.860\\
 & {} & {} & {}[0.267, 2.682]\\
Asian:Age.L & {} & {} & 1.267\\
 & {} & {} & {}[0.984, 1.630]\\
Black:Age.L & {} & {} & 1.294\\
 & {} & {} & {}[0.735, 2.322]\\
Indian:Age.L & {} & {} & 1.203\\
 & {} & {} & {}[0.820, 1.776]\\
Indigenous:Age.L & {} & {} & 1.464\\
 & {} & {} & {}[0.530, 4.390]\\
Latine:Age.L & {} & {} & 1.339\\
 & {} & {} & {}[0.815, 2.242]\\
Multiracial:Age.L & {} & {} & 0.871\\
 & {} & {} & {}[0.319, 2.346]\\
RaceOther:Age.L & {} & {} & 0.999\\
 & {} & {} & {}[0.323, 3.174]\\
Asian:Phase2 & {} & {} & 2.175\\
 & {} & {} & {}[1.133, 4.388]\\
Black:Phase2 & {} & {} & 2.060\\
 & {} & {} & {}[1.499, 2.833]\\
Indian:Phase2 & {} & {} & 0.998\\
 & {} & {} & {}[0.043, 27.924]\\
Indigenous:Phase2 & {} & {} & 2.801\\
 & {} & {} & {}[0.664, 15.780]\\
Latine:Phase2 & {} & {} & 1.789\\
 & {} & {} & {}[1.364, 2.359]\\
Multiracial:Phase2 & {} & {} & 1.000\\
 & {} & {} & {}[0.036, 24.168]\\
RaceOther:Phase2 & {} & {} & 0.437\\
 & {} & {} & {}[0.128, 1.328]\\
Asian:Phase3 & {} & {} & 1.847\\
 & {} & {} & {}[0.985, 3.604]\\
Black:Phase3 & {} & {} & 1.694\\
 & {} & {} & {}[1.301, 2.190]\\
Indian:Phase3 & {} & {} & 3.250\\
 & {} & {} & {}[1.860, 5.725]\\
Indigenous:Phase3 & {} & {} & 2.330\\
 & {} & {} & {}[0.680, 9.821]\\
Latine:Phase3 & {} & {} & 1.458\\
 & {} & {} & {}[1.103, 1.929]\\
Multiracial:Phase3 & {} & {} & 0.809\\
 & {} & {} & {}[0.210, 2.754]\\
RaceOther:Phase3 & {} & {} & 0.982\\
 & {} & {} & {}[0.042, 22.561]\\
sd\_dialogue\_id\_\_Intercept & 2.439 & 2.376 & 2.378\\
 & {}[2.351, 2.534] & {}[2.295, 2.471] & {}[2.298, 2.472]\\
sd\_rater\_id\_\_Intercept & 2.329 & 2.463 & 2.251\\
 & {}[2.169, 2.539] & {}[2.251, 2.739] & {}[2.073, 2.472]\\
%\midrule
%Num.Obs. & 101286 & 85596 & 85596\\
%N rater_id  &   252 &   209 &   209\\
%N dialogue_id   &   1340    &   1340    &   1340\\
%R2 & 0.409 & {} & {}\\
%R2 Marg. & 0.000 & {} & {}\\
%ICC & 0.6 & {} & {}\\
%ELPD & -56411.5 & -47373.9 & -47348.4\\
%ELPD s.e. & 242.4 & 223.4 & 223.4\\
%LOOIC & 112823.1 & 94747.9 & 94696.7\\
%LOOIC s.e. & 484.7 & 446.7 & 446.8\\
%WAIC & 112814.7 & 94737.6 & 94686.3\\
%\bottomrule
\end{tabular}
\caption{Summary of results for MLMs with recruitment phase as a variable, but no expert ratings.}
% \label{tab:summary-main-model}
\end{table}

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/bfit_v1v2v3_probit_8_priors_updated_race_phase_genx.png}
    \caption{Credible intervals for the AD intersectional model described in the \emph{Methods} section show that East and South Asian, and Indigenous raters, show strong differences in safety raters between data phases 1 and 2 than other raters. }
    \label{fig:race_genx}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=.45\textwidth]{figures/bfit_v1v2v3_probit_8_priors_updated_race_phase_genz.png}
    \caption{Credible intervals for the AD intersectional model described in the \emph{Methods} section show that East and South Asian, and Indigenous raters, show strong differences in safety raters between data phases 1 and 2 than other raters.}
    \label{fig:race_genz}
\end{figure}



\begin{table}[h!]
\begin{tabular}{r|dc}
\footnotesize
 Variable &  {Odds} & {95\% Credible Interval} \\
\hline
Intercept[1]  & 2.151 
 &  {}[1.550, 2.989]\\
Intercept[2] &  2.774
 & {}[1.995, 3.849]\\
Asian & 1.298
 & {}[0.740, 2.236]\\
Black &  1.233
 &  {}[0.704, 2.141]\\
Indian &  1.766
  & {}[1.130, 2.796]\\
Indigenous & 2.044
  & {}[0.906, 4.711]\\
Latine  & 1.410
 & {}[0.446, 4.849]\\
Multiracial & 1.410
 &  {}[0.671, 3.008]\\
RaceOther & 1.663
 & {}[0.736, 3.832]\\
Nonbinary & 0.923
 &  {}[0.149, 5.429]\\
Self-Described &  0.980
 &  {}[0.042, 21.433]\\
Woman  & 1.163
 &  {}[0.771, 1.727]\\
Age.L & 0.551
 & {}[0.442, 0.689]\\
Severity.L &  1.482
 & {}[1.281, 1.713]\\
Highschoolorbelow & 0.929
 &  {}[0.670, 1.304]\\
EducationOther & 0.949
 & {}[0.514, 1.735]\\
Asian:Woman & 0.485
 & {}[0.240, 0.969]\\
Black:Woman  & 0.858
 & {}[0.417, 1.766]\\
Indian:Woman & 1.668
 & {}[0.926, 3.030]\\
Indigenous:Woman & 1.210
 & {}[0.403, 3.759]\\
Latine:Woman & 1.276
 & {}[0.396, 4.049]\\
Multiracial:Woman & 1.134
 & {}[0.419, 3.038]\\
RaceOther:Woman & 0.905
 & {}[0.291, 2.799]\\
Asian:Age.L & 1.657
 & {}[1.256, 2.193]\\
Black:Age.L & 1.589
 & {}[0.857, 2.958]\\
Indian:Age.L & 1.280
 & {}[0.859, 1.980]\\
Indigenous:Age.L & 1.633
 & {}[0.540, 5.320]\\
Latine:Age.L & 0.901
 & {}[0.126, 6.249]\\
Multiracial:Age.L & 1.186
 & {}[0.471, 2.975]\\
RaceOther:Age.L & 1.189
 & {}[0.357, 4.029]\\
Asian:Severity.L & 1.036
 & {}[0.897, 1.200]\\
Black:Severity.L & 0.986
 & {}[0.869, 1.117]\\
Indian:Severity.L & 1.096
 & {}[0.966, 1.247]\\
Indigenous:Severity.L & 1.259
 & {}[1.033, 1.529]\\
Latine:Severity.L & 1.151
 & {}[0.901, 1.463]\\
Multiracial:Severity.L & 1.009
 & {}[0.848, 1.203]\\
RaceOther:Severity.L & 0.889
 & {}[0.674, 1.175]\\
conversation\_id\_\_Inter  & 2.075
 & {}[1.988, 2.171]\\
sd\_rater\_id\_Intercept & 2.344
 &  {}[2.134, 2.616]\\
sd\_rater\_id\_Sever.L & 1.167
  & {}[1.106, 1.233]\\
cor\_rater\_id\_Inter\_Sever.L  & 0.993
& {}[0.718, 1.380]\\
%\midrule
%Num.Obs. & 56468 & 42148 & 42148 & 42148\\
%R2 & 0.378 & 0.380 & 0.384 & 0.385\\
%R2 Marg. & 0.000 & 0.130 & 0.127 & 0.135\\
%ICC & 0.6 & {} & {} & {}\\
%ELPD & -35303.1 & -26553.5 & -26514.2 & -26509.1\\
%ELPD s.e. & 178.4 & 154.5 & 154.6 & 154.8\\
%LOOIC & 70606.2 & 53107.1 & 53028.5 & 53018.1\\
%LOOIC s.e. & 356.8 & 309.0 & 309.1 & 309.6\\
%WAIC & 70602.7 & 53103.1 & 53023.0 & 53012.4\\
\end{tabular}
\caption{Summary of results for MLMs of Expert-Annotated Data. These results show the estimated odds according to the model for the class in question versus the variable's reference class that the conversation being rated \emph{safe}. Note that, for gender \emph{Man} is the reference class, for race/ethnicity it is \emph{White}, for dataset phase it is \emph{phase 1}, and for age it is \emph{Gen Z}.}
\label{tab:expert}
\end{table}

\begin{table}
\centering
\begin{tabular}[h!]{r|dc}
\footnotesize
 Variable & {Odds} & 95\% Credible Interval \\
\hline
Intercept[1]  & 3.037
 &  {}[2.221, 4.198]\\
Intercept[2] & 3.915
& {}[2.860, 5.404]\\
Asian & 0.985
 &  {}[0.489, 1.966]\\
Black & 0.826
 &  {}[0.480, 1.432]\\
Indian & 1.256
 &  {}[0.812, 1.950]\\
Indigenous & 1.436
 &  {}[0.611, 3.442]\\
Latine & 0.937
 &  {}[0.554, 1.566]\\
Multiracial & 1.628
 & {}[0.510, 6.072]\\
RaceOther & 2.760
 & {}[0.964, 8.811]\\
Woman & 1.226
 & {}[0.840, 1.801]\\
Age.L & 0.650
 & {}[0.548, 0.771]\\
Highschoolorbelow & 1.148
 & {}[0.846, 1.558]\\
EducationOther & 0.688
 &  {}[0.373, 1.255]\\
Phase2 & 0.692
 & {}[0.606, 0.792]\\
Phase3 &  1.418
 &  {}[1.179, 1.705]\\
Asian:Woman  & 0.457
  & {}[0.232, 0.875]\\
Black:Woman  & 0.785
  & {}[0.388, 1.567]\\
Indian:Woman  & 1.654
  & {}[0.931, 2.942]\\
Indigenous:Woman  & 1.046
  & {}[0.327, 3.413]\\
Latine:Woman  & 0.907
  & {}[0.487, 1.724]\\
Multiracial:Woman  & 0.982
  & {}[0.363, 2.685]\\
RaceOther:Woman  & 0.860
  & {}[0.267, 2.682]\\
Asian:Age.L  & 1.267
  & {}[0.984, 1.630]\\
Black:Age.L  & 1.294
  & {}[0.735, 2.322]\\
Indian:Age.L  & 1.203
  & {}[0.820, 1.776]\\
Indigenous:Age.L  & 1.464
  & {}[0.530, 4.390]\\
Latine:Age.L  & 1.339
  & {}[0.815, 2.242]\\
Multiracial:Age.L  & 0.871
  & {}[0.319, 2.346]\\
RaceOther:Age.L  & 0.999
  & {}[0.323, 3.174]\\
Asian:Phase2  & 2.175
  & {}[1.133, 4.388]\\
Black:Phase2  & 2.060
  & {}[1.499, 2.833]\\
Indian:Phase2  & 0.998
  & {}[0.043, 27.924]\\
Indigenous:Phase2  & 2.801
  & {}[0.664, 15.780]\\
Latine:Phase2  & 1.789
  & {}[1.364, 2.359]\\
Multiracial:Phase2  & 1.000
  & {}[0.036, 24.168]\\
RaceOther:Phase2  & 0.437
  & {}[0.128, 1.328]\\
Asian:Phase3  & 1.847
  & {}[0.985, 3.604]\\
Black:Phase3  & 1.694
  & {}[1.301, 2.190]\\
Indian:Phase3  & 3.250
  & {}[1.860, 5.725]\\
Indigenous:Phase3  & 2.330
  & {}[0.680, 9.821]\\
Latine:Phase3  & 1.458
  & {}[1.103, 1.929]\\
Multiracial:Phase3  & 0.809
  & {}[0.210, 2.754]\\
RaceOther:Phase3  & 0.982
  & {}[0.042, 22.561]\\
conversation\_id\_\_Intercept & 2.378
 &  {}[2.298, 2.472]\\
rater\_id\_\_Intercept & 2.251
 & {}[2.073, 2.472]
%\midrule
%Num.Obs. & 101286 & 85596 & 85596\\
%N rater_id  &   252 &   209 &   209\\
%N conversation_id   &   1340    &   1340    &   1340\\
%R2 & 0.409 \\
%R2 Marg. & 0.000 & {} & {}\\
%ICC & 0.6 & {} & {}\\
%ELPD & -56411.5 & -47373.9 & -47348.4\\
%ELPD s.e. & 242.4 & 223.4 & 223.4\\
%LOOIC & 112823.1 & 94747.9 & 94696.7\\
%LOOIC s.e. & 484.7 & 446.7 & 446.8\\
%WAIC & 112814.7 & 94737.6 & 94686.3\\
%\bottomrule
\end{tabular}
\caption{Summary of results for the MLM with data collection phase as a variable, but no expert ratings. These results show the estimated odds according to the model for the class in question versus the variable's reference class that the conversation being rated \emph{safe}. Note that, for gender  \emph{Man} is the reference class, for race/ethnicity it is \emph{White}, for dataset phase it is \emph{phase 1}, and for age it is \emph{Gen Z}.}
\label{tab:phase}
\end{table}





\begin{table*}
\footnotesize
\begin{tabular}{lllllllll}
\toprule
Row &                       Parameter &     Median & 95-CI-Lower & 95-CI-Upper & Direction & Significance & Large &   I \\
\midrule
  1 &                      Intercept1 &       1.11 &         0.8 &        1.43 &         1 &            1 &     1 &  ** \\
  2 &                      Intercept2 &       1.36 &        1.05 &        1.69 &         1 &            1 &     1 &  ** \\
  3 &                           Asian &      -0.01 &       -0.72 &        0.68 &      0.52 &         0.46 &  0.21 &     \\
  4 &                           Black &      -0.19 &       -0.73 &        0.36 &      0.75 &         0.69 &  0.35 &     \\
  5 &                          Indian &       0.23 &       -0.21 &        0.67 &      0.84 &         0.78 &  0.38 &   * \\
  6 &                      Indigenous &       0.36 &       -0.49 &        1.24 &      0.81 &         0.77 &  0.56 &   * \\
  7 &                         Latinxe &      -0.07 &       -0.59 &        0.45 &       0.6 &         0.53 &  0.19 &     \\
  8 &                     Multiracial &       0.49 &       -0.67 &         1.8 &      0.79 &         0.77 &  0.62 &     \\
  9 &                           Other &       1.02 &       -0.04 &        2.18 &      0.97 &         0.96 &  0.91 &  ** \\
 10 &                       Nonbinary &      -0.02 &       -1.92 &        1.78 &      0.51 &         0.48 &  0.37 &     \\
 11 &              SelfMdescribebelow &      -0.73 &       -2.52 &           1 &      0.81 &          0.8 &   0.7 &   * \\
 12 &                           Woman &        0.2 &       -0.17 &        0.59 &      0.86 &         0.79 &  0.32 &   * \\
 13 &                           age.L &      -0.43 &        -0.6 &       -0.26 &         1 &            1 &  0.94 &  ** \\
 14 &                           age.Q &       0.19 &       -0.16 &        0.55 &      0.85 &         0.78 &  0.28 &   * \\
 15 &                          Phase2 &      -0.37 &        -0.5 &       -0.23 &         1 &            1 &  0.83 &  ** \\
 16 &                          Phase3 &       0.35 &        0.16 &        0.53 &         1 &            1 &  0.69 &  ** \\
 17 &               Highschoolorbelow &       0.14 &       -0.17 &        0.44 &      0.81 &         0.71 &  0.15 &   * \\
 18 &                           Other &      -0.37 &       -0.99 &        0.23 &      0.89 &         0.86 &   0.6 &   * \\
 19 &                 Asian:Nonbinary &  -6.09E-03 &        -3.2 &        3.22 &       0.5 &         0.48 &   0.4 &     \\
 20 &                 Black:Nonbinary &       0.02 &        -3.2 &        3.07 &       0.5 &         0.49 &   0.4 &     \\
 21 &                Indian:Nonbinary &   1.48E-03 &       -3.12 &        3.24 &       0.5 &         0.48 &  0.39 &     \\
 22 &            Indigenous:Nonbinary &      -0.03 &       -1.89 &         1.9 &      0.51 &         0.49 &  0.37 &     \\
 23 &               Latinxe:Nonbinary &   2.63E-04 &       -3.28 &        3.17 &       0.5 &         0.48 &  0.39 &     \\
 24 &           Multiracial:Nonbinary &   6.84E-03 &       -3.16 &        3.31 &       0.5 &         0.48 &  0.39 &     \\
 25 &                 Other:Nonbinary &      -0.01 &       -3.12 &        3.24 &       0.5 &         0.49 &  0.39 &     \\
 26 &        Asian:SelfMdescribebelow &   4.78E-03 &       -3.22 &         3.1 &       0.5 &         0.48 &   0.4 &     \\
 27 &        Black:SelfMdescribebelow &       0.02 &       -3.18 &        3.18 &      0.51 &         0.49 &  0.39 &     \\
 28 &       Indian:SelfMdescribebelow &       0.01 &       -3.26 &         3.2 &       0.5 &         0.49 &   0.4 &     \\
 29 &   Indigenous:SelfMdescribebelow &  -8.76E-03 &       -3.19 &        3.28 &       0.5 &         0.48 &   0.4 &     \\
 30 &      Latinxe:SelfMdescribebelow &      -0.73 &        -2.5 &        1.04 &      0.81 &          0.8 &   0.7 &   * \\
 31 &  Multiracial:SelfMdescribebelow &   5.12E-03 &       -3.24 &        3.29 &       0.5 &         0.48 &  0.39 &     \\
 32 &        Other:SelfMdescribebelow &      -0.03 &       -3.03 &        2.99 &      0.51 &         0.49 &   0.4 &     \\
 33 &                     Asian:Woman &      -0.78 &       -1.46 &       -0.13 &      0.99 &         0.99 &  0.92 &  ** \\
 34 &                     Black:Woman &      -0.24 &       -0.95 &        0.45 &      0.75 &         0.71 &  0.44 &     \\
 35 &                    Indian:Woman &        0.5 &       -0.07 &        1.08 &      0.96 &         0.94 &  0.76 &  ** \\
 36 &                Indigenous:Woman &       0.05 &       -1.12 &        1.23 &      0.53 &          0.5 &  0.33 &     \\
 37 &                   Latinxe:Woman &       -0.1 &       -0.72 &        0.54 &      0.62 &         0.56 &  0.26 &     \\
 38 &               Multiracial:Woman &      -0.02 &       -1.01 &        0.99 &      0.51 &         0.47 &  0.28 &     \\
 39 &                     Other:Woman &      -0.15 &       -1.32 &        0.99 &      0.61 &         0.57 &  0.39 &     \\
 40 &                     Asian:age.L &       0.24 &       -0.02 &        0.49 &      0.97 &         0.93 &  0.31 &  ** \\
 41 &                     Black:age.L &       0.26 &       -0.31 &        0.84 &      0.81 &         0.76 &  0.45 &   * \\
 42 &                    Indian:age.L &       0.18 &        -0.2 &        0.57 &      0.83 &         0.75 &  0.28 &   * \\
 43 &                Indigenous:age.L &       0.38 &       -0.63 &        1.48 &      0.77 &         0.74 &  0.56 &     \\
 44 &                   Latinxe:age.L &       0.29 &        -0.2 &        0.81 &      0.87 &         0.83 &  0.49 &   * \\
 45 &               Multiracial:age.L &      -0.14 &       -1.14 &        0.85 &       0.6 &         0.57 &  0.37 &     \\
 46 &                     Other:age.L &  -8.30E-04 &       -1.13 &        1.15 &       0.5 &         0.47 &   0.3 &     \\
 47 &                     Asian:age.Q &      -0.45 &       -1.23 &         0.3 &      0.89 &         0.86 &  0.65 &   * \\
 48 &                     Black:age.Q &      -0.44 &       -1.02 &        0.12 &      0.93 &         0.91 &  0.69 &  ** \\
 49 &                    Indian:age.Q &      -0.06 &       -0.68 &        0.57 &      0.57 &         0.51 &  0.22 &     \\
 50 &                Indigenous:age.Q &      -0.63 &       -2.04 &        0.59 &      0.84 &         0.82 &   0.7 &   * \\
 51 &                   Latinxe:age.Q &      -0.45 &       -1.03 &        0.12 &      0.94 &         0.91 &   0.7 &  ** \\
 52 &               Multiracial:age.Q &      -0.51 &       -1.46 &        0.39 &      0.86 &         0.84 &  0.67 &   * \\
 53 &                     Other:age.Q &      -1.15 &       -2.37 &       -0.07 &      0.98 &         0.98 &  0.94 &  ** \\
 54 &                    Asian:Phase2 &       0.78 &        0.12 &        1.48 &      0.99 &         0.99 &  0.93 &  ** \\
 55 &                    Black:Phase2 &       0.72 &         0.4 &        1.04 &         1 &            1 &  0.99 &  ** \\
 56 &                   Indian:Phase2 &  -1.53E-03 &       -3.14 &        3.33 &       0.5 &         0.48 &  0.39 &     \\
 57 &               Indigenous:Phase2 &       1.03 &       -0.41 &        2.76 &      0.92 &          0.9 &  0.83 &  ** \\
 58 &                  Latinxe:Phase2 &       0.58 &        0.31 &        0.86 &         1 &            1 &  0.98 &  ** \\
 59 &              Multiracial:Phase2 &  -4.30E-04 &       -3.33 &        3.19 &       0.5 &         0.48 &  0.39 &     \\
 60 &                    Other:Phase2 &      -0.83 &       -2.06 &        0.28 &      0.93 &         0.91 &  0.82 &  ** \\
 61 &                    Asian:Phase3 &       0.61 &       -0.01 &        1.28 &      0.97 &         0.96 &  0.84 &  ** \\
 62 &                    Black:Phase3 &       0.53 &        0.26 &        0.78 &         1 &            1 &  0.96 &  ** \\
 63 &                   Indian:Phase3 &       1.18 &        0.62 &        1.74 &         1 &            1 &     1 &  ** \\
 64 &               Indigenous:Phase3 &       0.85 &       -0.39 &        2.28 &      0.91 &          0.9 &   0.8 &  ** \\
 65 &                  Latinxe:Phase3 &       0.38 &         0.1 &        0.66 &         1 &         0.99 &  0.71 &  ** \\
 66 &              Multiracial:Phase3 &      -0.21 &       -1.56 &        1.01 &      0.63 &          0.6 &  0.45 &     \\
 67 &                    Other:Phase3 &      -0.02 &       -3.17 &        3.12 &      0.51 &         0.49 &   0.4 &     \\
\bottomrule
\end{tabular}

\caption{Results for the MLM Q\_overall $\sim$ race $*$ (gender $+$ age $+$ phase) $+$ education $+$ (1 $|$ rater\_id) $+$ (1 $|$ conversation\_id)}
\label{tab:bfit_v1v2v3_probit_8_priors_updated}
\end{table*}

\begin{table*}
    \centering
    \tiny
\begin{tabular}{lllllllll}
\toprule
Row &                       Parameter &     Median & 95-CI-Lower & 95-CI-Upper & Direction & Significance &     Large &   I \\
\midrule
  1 &                      Intercept1 &       0.79 &        0.44 &        1.12 &         1 &            1 &         1 &  ** \\
  2 &                      Intercept2 &       1.04 &        0.69 &        1.37 &         1 &            1 &         1 &  ** \\
  3 &                           Asian &        0.3 &       -0.26 &        0.86 &      0.85 &         0.81 &       0.5 &   * \\
  4 &                           Black &        0.2 &       -0.36 &        0.76 &      0.76 &          0.7 &      0.36 &     \\
  5 &                          Indian &       0.58 &        0.13 &        1.02 &      0.99 &         0.99 &      0.89 &  ** \\
  6 &                      Indigenous &       0.79 &       -0.02 &        1.64 &      0.97 &         0.96 &      0.89 &  ** \\
  7 &                         Latinxe &       0.27 &       -0.87 &        1.49 &      0.69 &         0.65 &      0.48 &     \\
  8 &                     Multiracial &       0.34 &        -0.4 &        1.11 &      0.82 &         0.78 &      0.55 &   * \\
  9 &                           Other &       0.51 &       -0.32 &        1.35 &      0.88 &         0.86 &      0.69 &   * \\
 10 &                       Nonbinary &      -0.14 &       -1.98 &        1.71 &      0.56 &         0.54 &      0.42 &     \\
 11 &              SelfMdescribebelow &      -0.01 &        -3.2 &        3.15 &       0.5 &         0.49 &      0.39 &     \\
 12 &                           Woman &       0.17 &       -0.25 &        0.59 &      0.79 &         0.72 &      0.28 &     \\
 13 &                           age.L &      -0.59 &       -0.82 &       -0.37 &         1 &            1 &         1 &  ** \\
 14 &                           age.Q &       0.21 &       -0.18 &        0.58 &      0.86 &          0.8 &      0.31 &   * \\
 15 &                degree\_of\_harm.L &       0.39 &        0.26 &        0.53 &         1 &            1 &      0.91 &  ** \\
 16 &                degree\_of\_harm.Q &      -0.41 &       -0.54 &       -0.27 &         1 &            1 &      0.94 &  ** \\
 17 &                degree\_of\_harm.C &       0.08 &       -0.07 &        0.22 &      0.85 &         0.63 &  7.50E-04 &   * \\
 18 &               Highschoolorbelow &      -0.02 &       -0.37 &        0.31 &      0.55 &         0.44 &      0.06 &     \\
 19 &                           Other &      -0.02 &       -0.63 &        0.59 &      0.53 &         0.46 &      0.19 &     \\
 20 &                 Asian:Nonbinary &   6.38E-03 &       -3.45 &        3.32 &       0.5 &         0.49 &       0.4 &     \\
 21 &                 Black:Nonbinary &  -4.64E-03 &       -3.02 &        3.13 &       0.5 &         0.48 &      0.39 &     \\
 22 &                Indian:Nonbinary &   6.95E-03 &       -3.14 &        3.14 &       0.5 &         0.48 &      0.39 &     \\
 23 &            Indigenous:Nonbinary &      -0.14 &       -2.05 &        1.63 &      0.56 &         0.54 &      0.42 &     \\
 24 &               Latinxe:Nonbinary &  -4.07E-03 &       -3.22 &        3.35 &       0.5 &         0.48 &      0.39 &     \\
 25 &           Multiracial:Nonbinary &      -0.01 &       -3.13 &        2.92 &       0.5 &         0.49 &      0.39 &     \\
 26 &                 Other:Nonbinary &      -0.02 &       -3.24 &        3.32 &      0.51 &         0.49 &       0.4 &     \\
 27 &        Asian:SelfMdescribebelow &       0.02 &       -3.15 &        3.09 &      0.51 &         0.49 &      0.39 &     \\
 28 &        Black:SelfMdescribebelow &   2.77E-03 &       -3.19 &        3.44 &       0.5 &         0.48 &      0.39 &     \\
 29 &       Indian:SelfMdescribebelow &      -0.01 &       -3.13 &        3.12 &      0.51 &         0.49 &      0.39 &     \\
 30 &   Indigenous:SelfMdescribebelow &  -3.36E-03 &       -3.11 &        3.16 &       0.5 &         0.48 &      0.39 &     \\
 31 &      Latinxe:SelfMdescribebelow &       0.02 &       -3.17 &        3.35 &      0.51 &         0.49 &       0.4 &     \\
 32 &  Multiracial:SelfMdescribebelow &   7.12E-03 &       -3.27 &        3.43 &       0.5 &         0.48 &       0.4 &     \\
 33 &        Other:SelfMdescribebelow &   4.26E-03 &       -3.02 &        3.29 &       0.5 &         0.48 &       0.4 &     \\
 34 &                     Asian:Woman &      -0.77 &       -1.48 &       -0.08 &      0.99 &         0.98 &      0.91 &  ** \\
 35 &                     Black:Woman &      -0.18 &       -0.89 &        0.57 &      0.69 &         0.64 &      0.37 &     \\
 36 &                    Indian:Woman &       0.52 &       -0.08 &        1.13 &      0.96 &         0.94 &      0.76 &  ** \\
 37 &                Indigenous:Woman &       0.11 &       -0.99 &        1.28 &      0.58 &         0.54 &      0.37 &     \\
 38 &                   Latinxe:Woman &       0.29 &       -0.84 &        1.48 &      0.69 &         0.66 &      0.49 &     \\
 39 &               Multiracial:Woman &       0.02 &          -1 &        1.05 &      0.51 &         0.48 &      0.29 &     \\
 40 &                     Other:Woman &      -0.11 &       -1.28 &        1.04 &      0.58 &         0.54 &      0.37 &     \\
 41 &                     Asian:age.L &       0.47 &        0.19 &        0.75 &         1 &            1 &      0.88 &  ** \\
 42 &                     Black:age.L &       0.41 &        -0.2 &        1.06 &      0.91 &         0.88 &      0.64 &  ** \\
 43 &                    Indian:age.L &       0.22 &       -0.19 &        0.63 &      0.85 &         0.79 &      0.35 &   * \\
 44 &                Indigenous:age.L &       0.34 &       -0.78 &         1.5 &      0.72 &         0.69 &      0.53 &     \\
 45 &                   Latinxe:age.L &      -0.06 &          -2 &        1.83 &0.53 &          0.5 &      0.39 &     \\
 46 &               Multiracial:age.L &       0.19 &       -0.76 &        1.16 &      0.66 &         0.62 &      0.42 &     \\
 47 &                     Other:age.L &       0.18 &       -1.03 &         1.4 &      0.62 &         0.58 &      0.42 &     \\
 48 &                     Asian:age.Q &       -0.8 &       -1.58 &       -0.02 &      0.98 &         0.97 &       0.9 &  ** \\
 49 &                     Black:age.Q &      -0.49 &       -1.09 &        0.12 &      0.94 &         0.92 &      0.72 &  ** \\
 50 &                    Indian:age.Q &       0.05 &       -0.62 &        0.72 &      0.55 &         0.49 &      0.23 &     \\
 51 &                Indigenous:age.Q &      -0.53 &       -1.93 &        0.73 &      0.79 &         0.76 &      0.63 &     \\
 52 &                   Latinxe:age.Q &      -0.32 &       -1.69 &        0.99 &      0.69 &         0.67 &      0.51 &     \\
 53 &               Multiracial:age.Q &       -0.5 &       -1.43 &         0.4 &      0.86 &         0.84 &      0.67 &   * \\
 54 &                     Other:age.Q &      -1.17 &       -2.45 &        0.03 &      0.97 &         0.97 &      0.92 &  ** \\
 55 &          Asian:degree\_of\_harm.L &       0.03 &       -0.09 &        0.14 &      0.67 &         0.34 &         0 &     \\
 56 &          Black:degree\_of\_harm.L &      -0.02 &       -0.12 &        0.08 &      0.62 &         0.25 &         0 &     \\
 57 &         Indian:degree\_of\_harm.L &       0.07 &       -0.04 &        0.18 &      0.91 &         0.65 &         0 &  ** \\
 58 &     Indigenous:degree\_of\_harm.L &       0.23 &        0.08 &        0.39 &         1 &         0.99 &      0.19 &  ** \\
 59 &        Latinxe:degree\_of\_harm.L &       0.11 &       -0.09 &        0.31 &      0.86 &         0.73 &      0.03 &   * \\
 60 &    Multiracial:degree\_of\_harm.L &  -6.33E-05 &       -0.14 &        0.14 &       0.5 &         0.25 &         0 &     \\
 61 &          Other:degree\_of\_harm.L &       -0.1 &       -0.32 &        0.13 &      0.81 &         0.67 &      0.04 &   * \\
 62 &          Asian:degree\_of\_harm.Q &       0.06 &       -0.04 &        0.18 &      0.89 &         0.61 &         0 &   * \\
 63 &          Black:degree\_of\_harm.Q &       0.07 &       -0.03 &        0.17 &      0.91 &         0.63 &         0 &  ** \\
 64 &         Indian:degree\_of\_harm.Q &       0.08 &       -0.02 &        0.18 &      0.94 &          0.7 &  8.33E-05 &  ** \\
 65 &     Indigenous:degree\_of\_harm.Q &      -0.08 &       -0.23 &        0.07 &      0.86 &         0.67 &  2.00E-03 &   * \\
 66 &        Latinxe:degree\_of\_harm.Q &       0.13 &       -0.07 &        0.34 &       0.9 &         0.79 &      0.05 &  ** \\
 67 &    Multiracial:degree\_of\_harm.Q &       0.02 &       -0.12 &        0.16 &      0.62 &         0.34 &  1.67E-04 &     \\
 68 &          Other:degree\_of\_harm.Q &       0.03 &        -0.2 &        0.27 &      0.61 &         0.45 &      0.01 &     \\
 69 &          Asian:degree\_of\_harm.C &       0.04 &       -0.07 &        0.16 &      0.78 &         0.46 &         0 &     \\
 70 &          Black:degree\_of\_harm.C &       0.05 &       -0.05 &        0.15 &      0.85 &         0.52 &         0 &   * \\
 71 &         Indian:degree\_of\_harm.C &       0.07 &       -0.03 &        0.18 &      0.92 &         0.68 &         0 &  ** \\
 72 &     Indigenous:degree\_of\_harm.C &       0.02 &       -0.13 &        0.18 &      0.61 &         0.37 &  4.17E-04 &     \\
 73 &        Latinxe:degree\_of\_harm.C &      -0.11 &       -0.32 &         0.1 &      0.86 &         0.72 &      0.04 &   * \\
 74 &    Multiracial:degree\_of\_harm.C &       0.03 &       -0.12 &        0.18 &      0.65 &          0.4 &  1.67E-04 &     \\
 75 &          Other:degree\_of\_harm.C &       0.13 &        -0.1 &        0.37 &      0.87 &         0.76 &      0.08 &   * \\
\bottomrule
\end{tabular}

    \caption{Q\_overall $\sim$ race * (gender + age + degree\_of\_harm) + education + (1 $|$ rater\_id) + (1 $|$ conversation\_id)}
    \label{tab:bfit_harm_4_priors_updated}
\end{table*}

